Erasure code-based low storage blockchain node

The concept of a decentralized ledger usually implies that each node of a blockchain network stores the entire blockchain. However, in the case of popular blockchains, which each weigh several hundreds of GB, the large amount of data to be stored can incite new or low-capacity nodes to run lightweight clients. Such nodes do not participate to the global storage effort and can result in a centralization of the blockchain by very few nodes, which is contrary to the basic concepts of a blockchain. To avoid this problem, we propose new low storage nodes that store a reduced amount of data generated from the blockchain by using erasure codes. The properties of this technique ensure that any block of the chain can be easily rebuild from a small number of such nodes. This system should encourage low storage nodes to contribute to the storage of the blockchain and to maintain decentralization despite of a globally increasing size of the blockchain. This system paves the way to new types of blockchains which would only be managed by low capacity nodes.

==> Makefile <==
#-----------------------------------------------------------------------------
# Basic parameters
#-----------------------------------------------------------------------------
# Softwares used. Please verify they are installed.
LATEX=pdflatex
LATEXMK=latexmk

# Target
ifeq ($(MAIN),)
MAIN=main
endif

#-----------------------------------------------------------------------------


#-----------------------------------------------------------------------------
# Advanced parameters
#-----------------------------------------------------------------------------
# LATEX options
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

# LATEXMK options
LATEXMKOPT=-pdf
CONTINUOUS=-pvc

SOURCES= $(shell find *.tex)
FIGURES := $(shell find images/* -type f)

#-----------------------------------------------------------------------------

#-----------------------------------------------------------------------------
# Makefile body
#-----------------------------------------------------------------------------
all: $(MAIN).pdf

.refresh:
	touch .refresh

$(MAIN).pdf: .refresh $(SOURCES) $(FIGURES)
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) $(NONSTOP) %O %S" $(MAIN)

force:
	touch .refresh
	rm $(MAIN).pdf
	$(LATEXMK) $(LATEXMKOPT) $(CONTINUOUS) \
		-pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out *.fdb_latexmk

once:
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

debug:
	$(LATEX) $(LATEXOPT) $(MAIN)

.PHONY: clean force once all

.PRECIOUS: $(MAIN).pdf

#-----------------------------------------------------------------------------

